SkelMamba: A State Space Model for Efficient Skeleton Action Recognition of Neurological Disorders

We introduce a novel state-space model (SSM)-based framework for skeleton-based human action recognition, with an anatomically-guided architecture that improves state-of-the-art performance in both clinical diagnostics and general action recognition tasks. Our approach decomposes skeletal motion analysis into spatial, temporal, and spatio-temporal streams, using channel partitioning to capture distinct movement characteristics efficiently. By implementing a structured, multi-directional scanning strategy within SSMs, our model captures local joint interactions and global motion patterns across multiple anatomical body parts. This anatomically-aware decomposition enhances the ability to identify subtle motion patterns critical in medical diagnosis, such as gait anomalies associated with neurological conditions. On public action recognition benchmarks, i.e., NTU RGB+D, NTU RGB+D 120, and NW-UCLA, our model outperforms current state-of-the-art methods, achieving accuracy improvements up to $3.2\%$ with lower computational complexity than previous leading transformer-based models. We also introduce a novel medical dataset for motion-based patient neurological disorder analysis to validate our method's potential in automated disease diagnosis.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
%\newcommand{\red}[1]{{\color{red}#1}}
%\newcommand{\todo}[1]{{\color{red}#1}}
%\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


==> sec/7_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> tables/sota_comparison_koa.tex <==
\begin{table}[t]
\centering
\caption{($\uparrow$ higher is better, $\downarrow$ lower is better).}
\label{tab:koa}
\footnotesize
\begin{tabularx}{\linewidth}{l X X X}
\toprule
 & $\modalityj$ & $\modalityjb$ & $\modalityjbm$ \\
\midrule
2S-AAGCN & 94.74 & 97.89 & 98.95 \\
PoseC3D & 98.95 & 100.00 & 100.00 \\
STGCN++ & 93.68 & 94.74 & 95.79 \\
Hyperformer & 100.00 & 100.00 & 97.89 \\
SkelMamba (Ours) & 100.00 & 100.00 & 100.00 \\
\bottomrule
\end{tabularx}
\end{table}




==> tables/sota_comparison_uniroma1.tex <==
\begin{table}[t]
\centering
\caption{($\uparrow$ higher is better, $\downarrow$ lower is better).}
\label{tab:uniroma1}
\footnotesize
\begin{tabularx}{\linewidth}{l X X X}
\toprule
 & $\modalityj$ & $\modalityjb$ & $\modalityjbm$ \\
\midrule
2S-AAGCN & 100.00 & 100.00 & 100.00 \\
PoseC3D & 84.79 & 89.40 & 89.86 \\
STGCN++ & 99.54 & 100.00 & 100.00 \\
Hyperformer & 98.62 & 99.54 & 99.54 \\
\bottomrule
\end{tabularx}
\end{table}




